HOIGPT: Learning Long Sequence Hand-Object Interaction with Language Models

We introduce HOIGPT, a token-based generative method that unifies 3D hand-object interactions (HOI) perception and generation, offering the first comprehensive solution for captioning and generating high-quality 3D HOI sequences from a diverse range of conditional signals (\eg text, objects, partial sequences). At its core, HOIGPT utilizes a large language model to predict the bidrectional transformation between HOI sequences and natural language descriptions. Given text inputs, HOIGPT generates a sequence of hand and object meshes; given (partial) HOI sequences, HOIGPT generates text descriptions and completes the sequences. To facilitate HOI understanding with a large language model, this paper introduces two key innovations: (1) a novel physically grounded HOI tokenizer, the hand-object decomposed VQ-VAE, for discretizing HOI sequences, and (2) a motion-aware language model trained to process and generate both text and HOI tokens. Extensive experiments demonstrate that HOIGPT sets new state-of-the-art performance on both text generation (+2.01% R Precision) and HOI generation (-2.56 FID) across multiple tasks and benchmarks.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/1.2_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
\vspace{-0.2in} 
\centering
\includegraphics[width=1\linewidth]{figs/teaser.pdf}
\vspace{-0.25in} 
\caption{HOIGPT can handle a variety of HOI motion-related tasks based on different text instructions. Examples include text-to-motion generation, motion completion given object movement, and motion captioning. HOIGPT generates or interprets HOI sequences in response to user queries, showcasing its capability to understand and produce contextually relevant HOI motions. 
% The sequences represent time order from left to right, with generated motions shown in response to the provided instructions.
}
\label{fig:teaser}
\vspace{-0.25in}
\end{figure}

Hand-object interaction (HOI) refers to how humans use one or both hands to directly manipulate objects, such as tool manipulations, skilled activities, and exploration tasks.
These actions are among the primary ways that humans interact with the physical world.
Thus, generating and understanding HOI in 3D is pivotal to advancing machine intelligence in human-centric and embodied applications, such as human activity understanding, AR/VR, and robotics. 

Intuitively, both generation and perception of HOI involve strong physical reasoning capabilities. However, despite great progress made in HOI generation and understanding, the community has been treating them as two separate problems. Methods often focus either on HOI generation from text~\cite{christen2024diffh2o, cha2024text2hoi, sohl2015deep} or focus on perceiving and classifying HOI with text labels~\cite{}. It's natural to ask: how do we build a unified system that models the bidrectional transformation between HOI and text?

In this paper, we answer this question by taking inspirations from a seemingly unrelated field in  foundation models, specifically large language models (LLMs)~\cite{devlin-etal-2019-bert, t5, dubey2024llama, achiam2023gpt}. With continuous breakthroughs over the years, LLMs nowadays demonstrates surprising reasoning abilities by generating long, coherent text messages in multi-turn dialogue. In addition, they have been proven to be an effective method to perceive, reason and generate multi-modal data. The reasoning abilities and multi-modal adaptability makes LLMs a promising universal interfaces for bidirectional transformation across modalities. 

Is it possible to adopt LLMs for modeling HOI that has strong physically grounded motion patterns?
Previous works~\cite{jiang2024motiongpt,zhang2024motiongpt, radosavovic2024humanoid, ribeiro2024motiongpt, wang2024motiongpt} have shown that human body motion can be perceived and generated through an LLM. These methods tokenizes the human motion data (e.g., using a VQVAE~\cite{van2017neural}) and fine-tune the LLM to interpret and generate these motion tokens as a novel ``language of motion". 

We follow a similar path by encoding HOI sequences into tokens. Different from tokenizing human body motions, tokenizing human-object interactions involve several unique yet interesting challenges. First, HOI involves complex interactions of multiple entities (two hands + objects) where human body motion is a single entity. This adds a layer of risks for physically implausible representations such as penetration or loss of contacts, which requires a next-level model physical reasoning abilities. Furthermore, while human bodies are largely similar, objects are very diverse; even more complex, each object has varying interaction patterns and affordances, leading to virtually limitless possibilities; this variability in objects contrasts with high conformities in human bodies and hands, which can often be parameterize with generic compact models~\cite{MANO, SMPL2015}.
The complex interplay between hands and objects and the objects' high diversity renders an enormous joint space of possible movements; naively tokenizing them following human motions perform poorly.

% In a seemingly unrelated field, large language models (LLMs) have made stunning advances in recent years \cite{devlin-etal-2019-bert, t5, dubey2024llama, achiam2023gpt}. 
% While not perfect, LLMs can now generate long, coherent text passages or even converse in multi-turn dialogue.
% Interestingly, LLMs have also proven highly compatible with modalities beyond text, demonstrating increasing viability as universal interfaces and raising the possibility of transferring the extensive knowledge distilled in LLMs to other modalities.
% The latter is particularly attractive for HOI due to the difficulty of data collection (and subsequent small scale of existing data). Other characteristics of multimodal LLMs, such as bidirectionality, descriptive abilities, flexible conditioning, and long-sequence coherence, pose a potential solution to a unified system for HOI understanding and generation.

To address these challenges, we propose \textbf{HOIGPT}, an autoregressive generative model designed for bidirectional transformations between 3D HOI motion and corresponding textual descriptions.
HOIGPT contains several key innovations.
Core to our work is a novel tokenizer tailored for HOI; it effectively factorizes HOI motion token space, reducing the the complex high-dimensional space to compact physically and semantically plausible space and improving generality. 
% while still enforcing physical and semantical constraints to 3D hand-object interactions—a challenge not present in single-entity human body motion yet critical for generating plausible and coherent long HOI sequences. 
With the HOI tokenizer, we propose a pretraining framework for HOI tokens that enables the language model to capture the relationships between various HOI tokens. The resulting model, HOIGPT, is capable for a suite of generation and understanding tasks, including HOI comprehension, generation, motion completion, and motion prediction—all using the same model. Our contributions are summarized as follows:
\begin{itemize}
    \item We introduce HOIGPT, the first unified model for bidirectional transformation between HOI motion and text descriptions, leveraging autoregressive language models. This approach enables a single model to understand and generate HOI motions and perform HOI motion prediction and completion.
    \item We present the HOI tokenizer, the first tokenizer designed to discretize HOI motions, addressing the lack of physical grounding in language tokens. Our approach incorporates novel geometric loss functions and a residual VQ-VAE architecture to enhance physical grounding.
    \item With these innovations, HOIGPT achieves state-of-the-art performance in both HOI generation and understanding, significantly outperforming all previous methods.
\end{itemize}

% Recent research, however, has primarily focused on generating HOI motion sequences from text using diffusion models~\cite{christen2024diffh2o, cha2024text2hoi, sohl2015deep}.
% LSuch models are capable of generating HOI motion sequences with realistic appearances, but they have certain shortcomings that prevent them from being applied in broader HOI settings. Besides lacking a bidirectionality feature for comprehension or description tasks, they exhibit: 1) limited flexibility in conditioning: Text prompts are often the only method of steering generation. This limits their ability to condition the motion as needed for motion completion, prediction, or blending. 2) limited to short sequences: Diffusion models struggle to generate coherent, longer sequences of motion, partially due to challenges in leveraging prior knowledge and enforcing temporal consistency.

% Solving such challenges is necessary for many broader HOI applications, unlocking needed capabilities.



% Recognizing the potential of combining large language models (LLMs) with motion data, several recent studies have utilized LLMs to model human body motion~\cite{jiang2024motiongpt,zhang2024motiongpt, radosavovic2024humanoid, ribeiro2024motiongpt, wang2024motiongpt}. These approaches involve tokenizing motion data (e.g., using a VQVAE~\cite{van2017neural}) and fine-tuning the LLM to interpret these motion tokens as a novel ``language.''
% A similar methodology can be applied to LLMs and HOI, but several challenges unique to HOI emerge.
% Chief among these is that while human body motion effectively models a single entity, HOI involves the interaction of up to three. Modeling these interactions requires a next-level reasoning ability in physical world.
% Furthermore, the set of possible objects in HOI is very diverse, each with varying interaction patterns and affordances, leading to virtually limitless possibilities; this variability in objects contrasts with human bodies and hands, which are often parameterizable with specialized and compact models~\cite{MANO, SMPL2015}.
% The complex interplay between hands and objects and the objects' high diversity results in an enormous joint space of possible movements, which naive tokenization implementations can struggle to model.


% In this paper, we propose \textbf{HOIGPT}, an autoregressive generative model designed for bidirectional transformations between 3D HOI motion and corresponding textual descriptions.
% HOIGPT contains several key innovations.
% Core to our work is a novel tokenizer specifically tailored for HOI that effectively factorizes HOI motion token space, reducing the required complexity and improving generality while still enforcing physical and semantical constraints to 3D hand-object interactions—a challenge not present in single-entity human body motion yet critical for generating plausible and coherent long HOI sequences. 
% We also propose a pretraining approach for HOI tokens that enables the language model to capture the relationships between various HOI tokens more effectively. This enables several downstream HOI generation and understanding tasks, including HOI comprehension, generation, motion completion, and motion prediction—all using the same model with different prompts.

% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We introduce HOIGPT, the first unified model for bidirectional transformation between HOI motion and text descriptions, leveraging autoregressive language models. This approach enables a single model to understand and generate HOI motions and perform HOI motion prediction and completion.
%     \item We present the HOI tokenizer, the first tokenizer designed to discretize HOI motions, addressing the lack of physical grounding in language tokens. Our approach incorporates novel geometric loss functions and a residual VQ-VAE architecture to enhance physical grounding.
%     \item With these innovations, HOIGPT achieves state-of-the-art performance in both HOI generation and understanding, significantly outperforming all previous methods.
% \end{itemize}

% \begin{itemize}
%     \item We propose the first HOI tokenizer for converting hand-object interaction motions into discrete tokens: a hand-object residual vector quantization model that vector-quantizes multiple entities (hands and objects) by modeling their residuals in a supervised manner. This HOI tokenizer is trained with loss functions that encode geometric constraints, ensuring physically plausible reconstructions. \FC{maybe we can leave tokenizer details in the technical section?}
%     \item We propose HOIGPT, the first autoregressive model for bidirectional transformation between HOI motion and text descriptions. To enhance this capability, we introduce HOI-language pretraining, enabling the language model to capture the relationships between various HOI tokens more effectively.
%     \item HOIGPT achieves state-of-the-art performance in both HOI generation and understanding, outperforming all previous methods by a large margin.
% \end{itemize}


==> sec/1_intro_DONOTEDIT.tex <==
\section{Introduction}
\label{sec:intro}

\haotang{Generating and understanding hand and object interaction (HOI) is an important task pivotal to advancing machine capabilities in human-centric applications, such as human activity understanding, AR/VR, and robotics. 
However, major breakthroughs remain elusive, in part due to the difficulty of high-fidelity data capture and the subsequent relatively low amount of data available.
Recent advancements in large language models (LLMs) like GPT, Llama, T5, and BERT~\cite{devlin-etal-2019-bert} (cite) have increased the viability of language as a universal interface in multimodal contexts (\eg images, videos, and meshes CITE), while also raising the possibility of transferring the extensive knowledge distilled in pretrained language models.
In this context, LLMs represent enormous potential for HOI generation and understanding.
}
% significantly enhanced the integration of multimodal generation and understanding, encompassing various modality like images, videos, mesh etc. 
% This unification allows these models to process and generate content across multiple modalities, leveraging the extensive knowledge captured in pretrained language models. 
% Incorporating LLMs into HOI generation and understanding holds significant potential. 
However, modeling interactions between multiple subjects using discrete tokens like language remains a challenging area, and no prior work has yet explored this direction.

\haotang{Interest in generating hand-object interactions (HOI) from text has only recently emerged, with a primary focus on diffusion-based approaches. \cite{christen2024diffh2o, cha2024text2hoi}. Despite their ability to generate realistic-looking hand-object interaction (HOI) motions, these diffusion-based methods face some limitations when compared to LLM-based generative approaches: 1) lack of bidirectional understanding. Diffusion-based methods typically lack the capability to interpret or generate textual descriptions from motion sequences. This unidirectional focus limits their utility in tasks that require comprehension and synthesis across modalities, such as translating observed motions into descriptive text. 2) limited control flexibility: These methods often support only a single type of control condition, such as text prompts, and struggle to incorporate additional control signals like motion completion, prediction, or blending. This limited flexibility restricts their adaptability and the precision of generated interactions, especially for complex HOI tasks requiring varied input conditions; 3) inability to generate long sequences: Diffusion models tend to produce shorter sequences, lacking the extended sequence-generation capabilities seen in large language models (LLMs). Without leveraging the prior knowledge and temporal consistency of LLM-inspired architectures, diffusion models are less effective at generating coherent, extended sequences necessary for realistic, sustained HOI motions.}

\haotang{Although extensive research has been conducted on generating human motion using large language models (LLMs) \cite{jiang2024motiongpt,zhang2024motiongpt}, modeling interactions between humans and objects is significantly more challenging, and no prior work has yet applied LLMs to this task. The primary challenge, compared to human motion generation, lies in modeling the additional interactions between the hand and object, which significantly increases the complexity of the task. To enable a language model to process HOI interactions and motion, raw HOI data must be converted into discrete sequences of motions and interactions using VQ-VAE, similar to other modalities (cite). These tokens are then fed into the language model along with corresponding text descriptions, allowing it to learn the correspondence between HOI and text, as well as the syntax and grammar of HOI tokens. Motion tokenization has been largely addressed in previous works, such as MotionGPT \cite{jiang2024motiongpt}. However, directly applying the same tokenization strategy to interactions does not work effectively, primarily due to the complex interplay between hands and objects, resulting in a large joint space of possible movements. Straightforward tokenization fails to enforce physically and semantically plausible 3D hand-object interactions—a challenge not present in single human motion. Additionally, the diversity of objects for interaction and their affordances is virtually unlimited, contrasting with human body or hand movements, which are often parameterized using specialized models like SMPL \cite{SMPL2015} or MANO \cite{MANO}. These factors highlight the need for a newly designed tokenizer specifically tailored for HOI, as well as a novel factorization approach to effectively address these complexities.}

\haotang{In this paper, we propose HOI-GPT, an autoregressive generative model designed to achieve bidirectional transformations between HOI motion and corresponding textual descriptions. By training HOI-GPT for both HOI generation and understanding, this approach enables a wide range of applications—including HOI comprehension, generation, motion completion, and motion prediction—all using the same model with different prompts. At the core of this work lie a newly designed HOI tokenizer and a pretraining approach utilizing HOI tokens. The HOI tokenizer employs object conditioning and a dual-decoder structure to model both the independent movement of different entities and their interplay for plausible joint motion. The careful arrangement of HOI tokens from different entities during language pretraining ensures that the language model can more effectively capture the relationships between various HOI tokens.}

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose the first HOI tokenizer for converting hand-object interaction motions into discrete tokens: a hand-object residual vector quantization model that vector-quantizes multiple entities (hands and object) by modeling their residuals in a supervised manner. This HOI tokenizer is trained with loss functions that encode geometric constraints, ensuring physically plausible reconstructions.
    % \item The proposed HOI tokenizer was trained with losses that garantuess the encodes geometric constraints to enforce physically plausible reconstruction.
    \item We propose HOI-GPT, the first autoregressive model for bidirectional transformation between HOI motion and text descriptions. To enhance this capability, we introduce HOI-language pretraining, enabling the language model to more effectively capture the relationships between various HOI tokens.
    \item HOI-GPT achieves state-of-the-art performance in both HOI generation and understanding, outperforming all previous methods by large margin.

\end{itemize}

\haotang{@mingzhen please check for correctness.}

% Hand-object interaction (HOI) are a common occurrence in our daily routines, involving the use of one or both hands to directly manipulate objects or utilize various tools. 
% These interactions play a crucial role in humans' ability to perform manipulation tasks effectively, acquire new skills, and adapt to ever-changing environments. 
Hand-object interaction (HOI) refers to how humans use one or both hands to directly manipulate objects, including for tool manipulation, skilled activity, or exploration purposes.
These kinds of actions are among the primary ways that humans affect action in the world. HOI is thus key to many wide-ranging applications, including human activity understanding, AR/VR interaction, and robotics.



For these reasons, there has been growing interest in understanding and generating HOI sequences~\cite{cha2024text2hoi, christen2024diffh2o}. \kjl{HOI-GPT is bidirectional, so it seems like we should also highlight that model that convert motion sequence to text is also valuable here.}
Several recent works take advantage of the latest advances in diffusion models~\cite{ho2020denoising} to generate a HOI sequence solely from text prompt. However, diffusion-based generative methods. Moreover, limited by diffusion models itself, those methods cannot generate text description given an arbitrary HOI motion.
\kjl{Why not use diffusion? What are the disadvantages? The motivation for why an LLM-based approach needs to be clearer}
% However, conditional HOI synthesis remains a challenge, as it requires the model to handle multimodal inputs and outputs 
\kjl{(Why? Is this something diffusion can't do?)}. 

Recent works on human motion generation~\cite{zhang2024motiongpt} leverage LLMs~\cite{touvron2023llama} to generate human pose conditioned on multimodal inputs where a VQVAE~\cite{van2017neural} is trained to tokenize the motion and then use it to finetune the language model along with text tokens. \kjl{Need to add explanation here why we want to take inspiration, and why it's superior to previous HOI approaches.}

We observe that this framework of casting human body motion as a token sequence learning problem for a language model can also apply to HOI, but a naive implementation will lead to underperformance due to the specific characteristics of HOI. 
In a human body pose sequence, there is ultimately only one entity, but in HOI, the movement and interplay between two hands can be fairly independent, resulting in a large joint space of possible movements.
Furthermore, the types of possible objects for interaction are virtually limitless; this diversity in objects contrasts with human bodies and hands, which are often parameterized with specialized models~\cite{MANO, SMPL2015}.

\kjl{Add paragraph more or less saying that naively modeling can be challenging. 
We propose a factorization foo.}

% Different from human motion generation, HOI involves a complicated interaction between hand-hand or hand-object, which present greater challenges for accurate modeling.

In this paper, we proposed HOI-GPT, a token-based autoregressive generative model to achieve bi-directional transformations between HOI motion and a corresponding text description. 
The main contributions of HOI-GPT can be summarized as follows:
\textcolor{cyan}{why using language model -> multi-action. first vqvae for the multiple subject and their interaction.}
\kjl{Some discussion of experiments to be added here.}
\begin{itemize}
    \item We propose HOI tokenizer: a hand-object residual vector quantization model that quantizes multiple subjects (hands and object) by modeling their residuals in a supervised manner.
    \item The proposed HOI tokenizer encodes geometric constraints to enforce physically plausible reconstruction.
    \item We proposed HOI-GPT, the first token-based model for bidirectional transformation between HOI motion and text descriptions in an autoregressive manner 

\end{itemize}
% Given the benefits bought from the natural of autoregressive method,
% One open question is: is LLM also able to handle the even more complex scenario of HOI generatation. In this proposal, we would like to explore if a LLMs-based HOI generator that is able to generate HOI and text from HOI and text conditioning.




==> sec/3.1_method_DONOTEDIT.tex <==
\section{Methodology}
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figs/Tokenization.pdf} \hskip 0.1in
\vspace{-2em}
\caption{ \textbf{Overview architecture for HOI tokenization.} The hand features are object feature are processed through the hand and object encoder. The encoded hand and object representations are learned with hand/object codebook and codebook-indices. The hand and object codebook-indices are learned separately for quantization of hand and objexct. The HOI latent code is subsequently decoded through the object and hand decoders to reconstruct the HOI sequence, producing a realistic hand-object interaction that aligns with the input features. Geometric loss is applied to ensure realistic hand-object interactions by minimizing interpenetration and maintaining plausible contact. }  % 
\label{fig:pipe}
\vspace{0.1in}
\end{figure*}

\subsection{Overview}
We propose HOI-GPT, a bidirectional text and HOI motion generative model.
As with other recent multimodal LLM works\cite{liu2023visual, moon2024anymal, jiang2024motiongpt}, we choose to unify both modalities in the text input token space, achieved by encoding HOI motion with a VQ-VAE (Sec.~\ref{sec:hoi_token}). 
A large-language model then reasons with this joint HOI and text representation (Sec.~\ref{sec:llm}), generating tokens that can be decoded as HOI motion or as text, depending on the task.
We impose several geometric regularizers during training of the VQ-VAE to ensure physical plausibility, and pre-train and instruction tune the LLM to learn to interpret the tokenized HOI motion~\ref{sec:training}.

\myheading{Hand-Object Representation}
We represent joint hand-object motion in 3D as a 6 degrees of freedom (6DoF) object pose and hand poses based on the MANO hand model~\cite{MANO}.  Specifically, object poses are defined as $\mO=\left(\tau_o, \phi_o, \alpha_o\right)$ where $\alpha_o$ denotes the object articulation angle, $\tau_o$ represents the global 3D object location, and $\phi_o$ is the 6D object rotation. Similarly, hand poses are expressed as $\mathcal{H}=\left(\boldsymbol{\tau}, \boldsymbol{\phi}\right)$, where $\boldsymbol{\tau}$ is the global 3D hand location, and $\phi$ refers to the 6D hand rotations, derived from the MANO~\cite{MANO}  parameters, which can also output hand vertices. The final HOI sequence are represented as $\mX_s = \texttt{concat}(\mO, \mH_l, \mH_r )$. 

\subsection{Residual HOI Tokenization} \label{sec:hoi_token}
Previous works on human motion synthesis compress and quantize the space of human actions into a codebook by learning a VQ-VAE~\cite{van2017neural}, effectively discretizing motion into tokens, which can then be passed to an LLM.
% However, when there are multiple entities, as in HOI, 
However, unlike for human body motion tokenizers, where the input space consists of the motions of a single entity, HOI involves up to three entities (two hands and an object). 
This requires careful network design to effectively encode tokenize multiple semi-independent entities and efficiently capture their complex interactions, without significantly ballooning the size of the requisite codebook.
% We further introduce a HOI tokenizer to convert HOI sequences into discrete tokens compatible with HOI-GPT's language model. 
In particular, we propose a multi-stage residual vector quantization (RVQ)~\cite{zeghidour2021soundstream} structure to capture fine-grained hand-object interactions, which we introduce below.

\myheading{HOI Encoder}. 
We start with two encoders: one for the object and one shared for both hands.
The hand encoder takes the hand pose $\mathcal{H}$ as input along with a hand type embedding to indicate the left or right hand. 
In parallel, an object encoder encodes the object pose, quantizing its spatial features and 6DoF pose; the canonical object point cloud is also encoded using PointNet~\cite{qi2017pointnet}, for object conditioning.
As a result, we obtain hands feature $\mZ_l$, $\mZ_r$, object feature $\mZ_o$ and canonical object conditioning $\C_o$.
These independent hand and objects features will then be fused into a shared latent space for a joint representation.
% The encoding process is structured in a hierarchical manner, where hand-object interaction (HOI) residuals are quantized in successive stages, to progressively refine the interaction details. 


\myheading{HOI Codebooks}. 
Standard VQ-VAEs represent the posterior distribution $q(z|x)$ by learning a single codebook, which indices query into in order to obtain the latent features.
% Different from a standard VQ-VAE that has a codebook and learns a posterior distribution $q(z|x)$ for indices to query the codebook and obtain the final latent feature, 
We instead introduce dual codebooks for hands and object, to separately model their motion patterns. As shown in \Fref{fig:pipe}, there are separate codebooks to represent the hand and object motion patterns. 
As motions by one hand can often be mirrored by the other, we use one hand codebook for both left and right hands; this allows the network to share learning of common patterns across hands. 
For queries, we learn three different queries for object, right hand, and left hand. 
The learned indices sequentially query the codebook to obtain the latent features, from object to right hand to left hand, resulting in the final HOI feature representation: $\mZ= \mZ_o + \mZ_l + \mZ_r + \C_o$. 
% \kjl{Is this a sum or just a set? The sequential decoding below doesn't seem possible if they've all been mixed together in a sum.} \MH{It is a sum, the object decoding takes only Z\_o as input}

\myheading{HOI Decoder}.
Our approach utilizes an object-conditioned HOI tokenization. For reconstruction, we also reconstruct the HOI conditioned on object motion. 
The object decoder $D_o$ first decodes features $\mZ_o + \C_o$ into object motion and further the predicted object motion and $\mZ$ are fed into the hand decoder to obtain the HOI motion. Such object conditioning ensures that the hand motion is conditioned on the object’s spatial and geometric properties. 
The final output HOI sequence $\hat{X}_s$ is thus:
\begin{equation}
    \hat{X}_s = D_h(\mZ | D_o(\mZ_o + \C_o))
\end{equation}





\subsection{HOI-aware Language Model} \label{sec:llm}
Our proposed method, HOI-GPT, integrates a novel residual VQ-VAE tokenization scheme with a language model to enable bidirectional transformation between Hand-Object Interactions (HOI) and natural language. 

\myheading{HOI tokens formulation}
Before training the language models, we first tokenize the HOI motion with our proposed HOI tokenizer. The residual tokenizer encodes each HOI sequence into discrete tokens that capture key aspects of the interaction. As a reminder, in our residual tokenization process, the hands and objects are separately tokenized with different queries where the query ids are used to form motion tokens in previous works~\cite{ribeiro2024motiongpt, jiang2024motiongpt}. Similarly, we form our hand object token as
$$
\langle \mathrm{HOI} \rangle \langle \mathrm{Hand}_i^{(L)} \rangle \langle \mathrm{Hand}_j^{(R)} \rangle \langle 
\mathrm{Object}_k \rangle \langle \backslash\mathrm{HOI} \rangle
$$
To achieve the bidirectional transformation, we combine the original text vocabulary along with HOI tokens to train our language models. This design enables the language model to process and learn from detailed motion information within the HOI sequence, capturing complex hand-object interactions and nuances.




\subsection{Training} \label{sec:training}

\myheading{HOI Tokenizer}.
% Next, the combined hand-object interaction is encoded, followed by a final step that quantizes the interactions involving both hands and the object. This step-by-step quantization--from object to hand-object and to hands-object--allows for detailed modeling of interaction dynamics. \BT{Do we show this as an ablation in the results?}
Our proposed HOI tokenizer incrementally learns the codebook indices for hands and objects to form a latent sequence. To accomplish this, we introduce a unique training strategy tailored for this purpose.
Following~\cite{van2017neural, zeghidour2021soundstream}, we incorporate reconstruction loss and latent embedding losses at each quantization stage. An embedding loss is calculated for each latent to ensure precise reconstruction of both hand and object motions. Different from RVQ~\cite{zeghidour2021soundstream}, benefit from our dual HOI encoder, our proposed method enforces the learning of residual in a supervised manner with the following embedding loss:

\begin{equation} \begin{aligned} 
\mathcal{L}_{\text{token}} = &|\m{X} - \hat{\m{X}}|_1 + \alpha \Big( |\mathbf{z}_o - \operatorname{sg}[\hat{\mathbf{z}}_o]|_2^2 \ + \\&|\mathbf{z}_o + \mathbf{z}_l - \operatorname{sg}[\hat{\mathbf{z}}_o + \hat{\mathbf{z}}_l]|_2^2 + |\mathbf{z} - \operatorname{sg}[\hat{\mathbf{z}}]|_2^2 \Big) 
\end{aligned} \end{equation}
where sg[$\cdot$] denotes the stop-gradient operation, and 
$\alpha$ is the weighting factor for the embedding constraint. This embedding loss is essential for minimizing reconstruction errors and maintaining the fidelity of complex interactions. By modeling these residuals independently, our proposed method effectively captures the nuances of hand-object dynamics, such as contact points and relative motion, making it highly effective for detailed HOI generation tasks.
To further enhance the robustness of HOI reconstruction, we follow the masking strategy from MAE~\cite{he2022masked}, where the hand or object latents are randomly masked. The masked latent is set to zero, diminishing its contribution. This design encourages each quantized latent for the hands or object to also learn correlations with the other, fostering stronger interactions between the components.

\myheading{Geometry-aware tokenization}. 
% The biggest challenge for generating HOI sequence is the physics implausible, e.g., the hand penetrates with the object. When tokenizing the HOI sequence, we also include additional 
Following previous works~\cite{hasson2019learning}, we introduce geometric constraints for understanding and generation of HOI while enforcing realistic physical interactions between hands and objects, minimizing unnatural penetrations while also maintaining natural contact between surfaces. 
We introduce three geometric losses below.

Following ~\cite{jiang2021hand}, we introduce the \textbf{Penetration Loss} \(L_{\text{penetr}}\) to penalize the predicted hand pose $\hat{\mH}$ where hand vertices penetrate the object’s surface. Given the prediction $\hat{\mH}$, we pass it into the MANO~\cite{MANO} to obtain the hand vertices $P$. For each hand vertex \( P \) inside the object, we find the closest object vertex \( {V}^o_i \) and minimize the squared distance \( \|P - {V}^o_i\|_2^2 \). The loss is averaged over all penetrating hand vertices to reduce unrealistic penetrations:
\begin{equation}
    \mL_{\text{pen}} = \frac{1}{|P_{\text{in}}^o|} \sum_{p \in P_{\text{in}}^o} \min_i \| p - \hat{V}_i \|_2^2
\end{equation}
where \( P_{\text{in}}^o \) represents the set of hand vertices inside the object.
\\
The \textbf{Contact Loss} $(\mL_C)$ enforces that hand joints stay within a specified distance \( \tau \) from the nearest object surface to maintain realistic interaction without gaps. Here, \( D(P_i^o) \) calculates the distance between hand vertices and the nearest object surfaces, and the constraint \( D(P_i^o) \leq \tau \) is imposed:
\begin{equation}
    \mL_C = \sum_{i} D(J_i^o), \quad \forall D(J_i^o) \leq \tau
\end{equation}
where \( D(J_i^o) = \min_j \| V_j^p - J_i^o \|_2^2 \), with \( V_j^p \) representing the object joints and \( J_i^o \) representing the hand joints. The contact loss would help generate a smooth hand motion before the hands contacting the object.
\\
The \textbf{Contact Region Loss} \(L_R\) promotes physically plausible contact by aligning ground truth hand vertices \( P_i^o \) at contact locations with corresponding reconstructed vertices \( p_i^o \). It minimizes the distance between the ground-truth hand vertices within a threshold distance \( \tau \) of the object surface and their reconstructed counterparts, ensuring that hand-object contact points are realistic by optimizing the predicted affordance region: \BT{Were there any other past works that do this? Would it be possible to claim this loss function as a novel contribution?} \MH{yes we could claim it}
\begin{equation}
    \mL_R = \sum_{i} \| P_i^o - \hat{P}_i^o \|_2, \quad \forall D(\hat{P}_i^o) \leq \tau    
\end{equation}
where \( \hat{P}_i^o \) represents ground truth hand vertices, \( P_i^o \) represents the reconstructed hand vertices, and \( D(\hat{P}_i^o) \) is the distance between the reconstructed hand vertices and the nearest object surface.
\\
The overall geometric loss is formulated as a weighted sum of those three losses:
    \begin{equation}
    \mL_{geo} = \lambda\mL_{pen} + \beta\mL_C + \gamma\mL_R    
\end{equation}
The geometric constraints improve the quality of hand-object interactions by penalizing unnatural penetrations, enforcing proximity between the hand and object before contacting, and ensuring contact at physically plausible regions.


\begin{figure}
\vspace{-0.2in} 
\centering
\includegraphics[width=1\linewidth]{figs/LLM.pdf}
\vspace{-0.25in} 
\caption{Language model training.}
\label{fig:llm}
\vspace{-2mm}
\end{figure}

\myheading{HOI tokenization loss function.} The final training objective function is formulated as:
    \begin{equation}
    \mL = \mL_{geo} + \mL_{token}
\end{equation}

\myheading{Language model}
During training, the input sequence $X_s = \{ x_s^i \}_{i=1}^N, x_s \in V$, is tokenized into a mixture of motion and language tokens, creating a unified vocabulary that allows the model to jointly handle both modalities. The target output sequence \( X_t = \{ x_t^i \}_{i=1}^L \) is predicted in an autoregressive manner, with the model learning to maximize the log-likelihood of the data distribution:

\begin{equation}
    \mathcal{L}_{lm} = - \sum_{i=0}^{L_t-1} \log p_\theta \left( x_t^i \mid x_t^{<i}, x_s \right).
\end{equation}

This framework allows HOI-GPT to learn complex relationships between motion and language, enabling flexible representation and generation of diverse hand-object interactions within a single model. Our method achieves state-of-the-art performance on multiple benchmarks, outperforming previous methods by a significant margin in both HOI generation from text and text generation from HOI motion.



==> sec/3_method_DONOTEDIT.tex <==

\section{Method}

\begin{figure*}[t]
% \vskip -0.2 in
\centering
\includegraphics[width=1.0\linewidth]{figs/Tokenization.pdf} \hskip 0.1in
% \vskip 0.1in
% \vskip -0.1 in
\vspace{-2em}
\caption{ \textbf{Overview architecture for HOI tokenization.} The hand features are object feature are processed through the hand and object encoder. The encoded hand and object representations are learned with hand/object codebook and codebook-indices. The hand and object codebook-indices are learned separately for quantization of hand and objexct. The HOI latent code is subsequently decoded through the object and hand decoders to reconstruct the HOI sequence, producing a realistic hand-object interaction that aligns with the input features. Geometric loss is applied to ensure realistic hand-object interactions by minimizing interpenetration and maintaining plausible contact. }  % 
\label{fig:pipe}
\vspace{0.1in}
\end{figure*}
 % \vspace{-2mm}
% Both \cite{zhang2024motiongpt} and our preliminary experimental results demonstrate that a VQVAE~\cite{van2017neural} codebook could well tokenize the human/hand motion, however, the tokenization of multiple object and their interaction still remains challenge.
\subsection{Hand-Object Representation}
% We represent joint hand-object motion in 3D as a 6 degrees of freedom (6DoF) object pose and hand poses using the MANO hand model~\cite{MANO}. More specifically, the object poses are defined as $\mO=\left(\tau_0, \phi_0, \alpha_o\right)$ where $\alpha_o$ is the object articulation angle, $\tau_0$ is the global 3D object location, and $\phi_0$ is the 6D object rotation. Similarly, the hand poses are defined as $\mathcal{H}_j=\left(\boldsymbol{\tau}, \boldsymbol{\phi}\right)$, where $\boldsymbol{\tau}$ is the global 3D hand objection location, and $\phi_0$ is the 6D object rotations which are MANO~\cite{MANO} hand pose parameters that could output the hand vertices.
We represent joint hand-object motion in 3D as a 6 degrees of freedom (6DoF) object pose and hand poses based on the MANO hand model~\cite{MANO}.  Specifically, object poses are defined as $\mO=\left(\tau_o, \phi_o, \alpha_o\right)$ where $\alpha_o$ denotes the object articulation angle, $\tau_o$ represents the global 3D object location, and $\phi_o$ is the 6D object rotation. Similarly, hand poses are expressed as $\mathcal{H}=\left(\boldsymbol{\tau}, \boldsymbol{\phi}\right)$, where $\boldsymbol{\tau}$ is the global 3D hand location, and $\phi$ refers to the 6D hand rotations, derived from the MANO~\cite{MANO}  parameters, which can also output hand vertices. The final HOI sequence are represented as $\mX_s = \texttt{concat}(\mO, \mH_l, \mH_r )$.
% \BT{Edited here a bit for clarity, please check for correctness, old paragraph commented.}


\subsection{Residual HOI Tokenization}
Previous works on human motion synthesis leverage a VQ-VAE~\cite{van2017neural} to learn the common pattern of human actions and further tokenize them. 
% However, when there are multiple entities, as in HOI, 
We further introduce a HOI tokenizer to convert HOI sequences into discrete tokens compatible with HOI-GPT's language model. Unlike traditional human motion tokenizers that process a single entity, HOI commonly involves up to three entities (two hands and an object). This requires careful network design to effectively encode and tokenize multiple entities and capture their complex interactions.

\myheading{HOI Encoder}. 
Our approach introduces a multi-stage residual vector quantization (RVQ)~\cite{zeghidour2021soundstream} structure to capture fine-grained hand-object interactions. This method employs separate encoders tailored to independently represent the hand and object features, which are then fused into a shared latent space for joint representation.
The encoding process is structured in a hierarchical manner, where hand-object interaction (HOI) residuals are quantized in successive stages, to progressively refine the interaction details. Initially, we have two encoders for hands and object separately where the hand encoder takes the hand pose $\mathcal{H}$ as as input along with hand type embedding to indict whether the hand pose is left hand or right hand. In the object encoder, we encode the object pose, quantizing its spatial features and 6DoF pose. 
We also encode the canonical object point cloud with PointNet~\cite{qi2017pointnet} as the object conditioning. As a result, we obtain hands feature $\mZ_l$, $\mZ_r$, object feature $\mZ_o$ and canonical object conditioning $\C_o$.

\myheading{HOI codebooks}. 
Different a standard VQ-VAE that has a codebook and learns a posterior distribution $q(z|x)$ for indices to query the codebook and obtain the final latent feature, 
we introduce a dual codebooks for hands and object to separately model their motions patterns. As shown in the \Fref{fig:pipe}, there are two codebook to represent the hand and object motion patterns. We use one hand codebook for both left and right hand as we find the left/right hands share common patterns and it is easier to learn such pattern. For queries, we also learn three different queries for object, right hand, left hands. The learned indices would query the the codebook to obtain the feature sequentially, from object to right hand to left hand. The final HOI feature representation $\mZ= \mZ_o + \mZ_l + \mZ_r + \C_o$.

\myheading{HOI Decoder}.
Our approach utilizes an object-conditioned HOI tokenization. For reconstruction, we also reconstruct the HOI conditioned on object motion. 
The object decoder $D_o$ would first decodes the $\mZ_o + \C_o$ to object motion and further the predicted object motion and $\mZ$ are fed into the hand decoder to obtain the HOI motion. Such object conditioning ensures that the hand motion is conditioned on the object’s spatial and geometric properties. 
The final output HOI sequence $\m\hat{X}_s$ would be:
\begin{equation}
    \m\hat{X}_s = D_h(\mZ | D_o(\mZ_o + \C_o))
\end{equation}

% Overall, the residual VQ-VAE is trained via a motion reconstruction loss combined with a latent embedding loss at each quantization layer


% \myheading{Object-conditioned HOI tokenization and reconstruction.}


% The tokenization process begins with independent encoders for the left hand, right hand, and object, which generate latent representations for each entity. These representations are then sequentially fused with object-specific features, ensuring that the hand motion is conditioned on the object’s spatial and geometric properties. Using a masking mechanism, the fused tokens guide the decoder in reconstructing both the object and hand motions separately before combining them to reconstruct the full HOI sequence. \kjl{Missing a discussion of the decoder architecture.} \BT{Do we have an ablation that shows that reconstructing first hand and object motions separately is better than reconstructing the complete hand and object motions jointly all at once? Might be good to justify the design choice above.}

% A geometric loss is applied as a constraint throughout this process to encourage accurate spatial alignment and prevent interpenetration between hands and objects, which are often physically implausible and visually jarring. This loss is particularly useful for preserving realistic contact points and natural hand-object positioning. Finally, the decoded outputs yield separate hand and object motion predictions, which are recombined to generate a realistic, interaction-consistent HOI reconstruction. This approach ensures that each HOI residual captures both independent hand movement and context-sensitive interaction dynamics, leading to improved hand-object interaction quality.

\myheading{Training HOI Tokenizer}.
% Next, the combined hand-object interaction is encoded, followed by a final step that quantizes the interactions involving both hands and the object. This step-by-step quantization--from object to hand-object and to hands-object--allows for detailed modeling of interaction dynamics. \BT{Do we show this as an ablation in the results?}
Our proposed HOI tokenizer incrementally learns the codebook indices for hands and objects to form a latent sequence. To accomplish this, we introduce a unique training strategy tailored for this purpose.
\\
Following~\cite{van2017neural, zeghidour2021soundstream}, we incorporate reconstruction loss and latent embedding losses at each quantization stage. An embedding loss is calculated for each latent to ensure precise reconstruction of both hand and object motions. Different with RVQ~\cite{zeghidour2021soundstream}, thanks to our dual HOI encoder, our porposed method enforces the learning of residual in a supervised manner with the following embedding loss:

\begin{equation} \begin{aligned} 
\mathcal{L}_{\text{token}} = &|\m{X} - \hat{\m{X}}|_1 + \alpha \Big( |\mathbf{z}_o - \operatorname{sg}[\hat{\mathbf{z}}_o]|_2^2 \ + \\&|\mathbf{z}_o + \mathbf{z}_l - \operatorname{sg}[\hat{\mathbf{z}}_o + \hat{\mathbf{z}}_l]|_2^2 + |\mathbf{z} - \operatorname{sg}[\hat{\mathbf{z}}]|_2^2 \Big) 
\end{aligned} \end{equation}
where sg[$\cdot$] denotes the stop-gradient operation, and 
$\alpha$ is the weighting factor for the embedding constraint. This embedding loss is essential for minimizing reconstruction errors and maintaining the fidelity of complex interactions. By modeling these residuals independently, our proposed method effectively captures the nuances of hand-object dynamics, such as contact points and relative motion, making it highly effective for detailed HOI generation tasks.
To further enhance the robustness of HOI reconstruction, we follow the masking strategy from MAE~\cite{he2022masked}, where the hand or object latents are randomly masked. The masked latent is set to zero, diminishing its contribution. This design encourages each quantized latent for the hands or object to also learn correlations with the other, fostering stronger interactions between the components.

\myheading{Geometry-aware tokenization}. 
% The biggest challenge for generating HOI sequence is the physics implausible, e.g., the hand penetrates with the object. When tokenizing the HOI sequence, we also include additional 
Following previous works~\cite{hasson2019learning} that modeling HOI with geometric contraints, we introduce the geometric constraints for understanding and generation HOI whles enforce realistic physical interactions between hands and objects, minimizing unnatural penetrations while also enforcing natural contact between surfaces. 
There are three geometric losses has been introduced here: \\
Following ~\cite{jiang2021hand}, we introduce the \textbf{Penetration Loss} \(L_{\text{penetr}}\) to penalize the predicted hand pose $\hat{\mH}$ where hand vertices penetrate the object’s surface. Given the prediction $\hat{\mH}$, we pass it into the MANO~\cite{MANO} to obtain the hand vertices $P$. For each hand vertex \( P \) inside the object, we find the closest object vertex \( {V}^o_i \) and minimize the squared distance \( \|P - {V}^o_i\|_2^2 \). The loss is averaged over all penetrating hand vertices to reduce unrealistic penetrations:
\begin{equation}
    \mL_{\text{pen}} = \frac{1}{|P_{\text{in}}^o|} \sum_{p \in P_{\text{in}}^o} \min_i \| p - \hat{V}_i \|_2^2
\end{equation}
where \( P_{\text{in}}^o \) represents the set of hand vertices inside the object.
\\
The \textbf{Contact Loss} $(\mL_C)$ enforces that hand joints stay within a specified distance \( \tau \) from the nearest object surface to maintain realistic interaction without gaps. Here, \( D(P_i^o) \) calculates the distance between hand vertices and the nearest object surfaces, and the constraint \( D(P_i^o) \leq \tau \) is imposed:
\begin{equation}
    \mL_C = \sum_{i} D(J_i^o), \quad \forall D(J_i^o) \leq \tau
\end{equation}
where \( D(J_i^o) = \min_j \| V_j^p - J_i^o \|_2^2 \), with \( V_j^p \) representing the object joints and \( J_i^o \) representing the hand joints. The contact loss would help generate a smooth hand motion before the hands contacting the object.
\\
The \textbf{Contact Region Loss} \(L_R\) promotes physically plausible contact by aligning ground truth hand vertices \( P_i^o \) at contact locations with corresponding reconstructed vertices \( p_i^o \). It minimizes the distance between the ground-truth hand vertices within a threshold distance \( \tau \) of the object surface and their reconstructed counterparts, ensuring that hand-object contact points are realistic by optimizing the predicted affordance region: \BT{Were there any other past works that do this? Would it be possible to claim this loss function as a novel contribution?} \MH{yes we could claim it}
\begin{equation}
    \mL_R = \sum_{i} \| P_i^o - \hat{P}_i^o \|_2, \quad \forall D(\hat{P}_i^o) \leq \tau    
\end{equation}
where \( \hat{P}_i^o \) represents ground truth hand vertices, \( P_i^o \) represents the reconstructed hand vertices, and \( D(\hat{P}_i^o) \) is the distance between the reconstructed hand vertices and the nearest object surface.
\\
The overall geometric loss is formulated as a weighted sum of those three losses:
    \begin{equation}
    \mL_{geo} = \lambda\mL_{pen} + \beta\mL_C + \gamma\mL_R    
\end{equation}
The geometric constraints improve the quality of hand-object interactions by penalizing unnatural penetrations, enforcing proximity between the hand and object before contacting, and ensuring contact at physically plausible regions.




\begin{figure}
\vspace{-0.2in} 
\centering
\includegraphics[width=1\linewidth]{figs/LLM.pdf}
\vspace{-0.25in} 
\caption{Language model training.}
\label{fig:llm}
\vspace{-0.25in}
\end{figure}
\subsection{HOI-awared Language Model}

% Following previous works, we use T5 as the, which is trained on natural language datasets.

Our proposed method, HOI-GPT, integrates a novel residual VQ-VAE tokenization scheme with a language model to enable bi-directional transformation between Hand-Object Interactions (HOI) and natural language. 

\myheading{HOI tokens formulation}
Before training the language models, we first tokenize the HOI motion with our proposed HOI tokenizer. The residual tokenizer encodes each HOI sequence into discrete tokens that capture key aspects of the interaction. Remind that with our residual tokenization process, the hands and objects are seperately tokenized with different queries where the query ids are used to form motion tokens in previous works~\cite{ribeiro2024motiongpt, jiang2024motiongpt}. Similarly, we form our hand object token as
% $< \text{  Token} \rangle \langle \text{Lhand\_Token\_i} \rangle \langle \text{Rhand\_Token\_j} \rangle \langle \text{Object\_Token\_k} \rangle \langle \text{HOI Token} \rangle$.
$$
\langle \text{HOI\_token} \rangle \langle \text{Lhand\_i} \rangle \langle \text{Rhand\_j} \rangle \langle 
\text{Object\_k} \rangle \langle \backslash\text{HOI\_token} \rangle
$$
To achieve the bi-directional tranformation, we combine the original text vocabulary along with HOI tokens to train our language models. This design enables the language model to process and learn from detailed motion information within the HOI sequence, capturing complex hand-object interactions and nuances.

\myheading{Language model training}
During training, the input sequence $X_s = \{ x_s^i \}_{i=1}^N$, is tokenized into a mixture of motion tokens $T_s$ and language tokens, creating a unified vocabulary that allows the model to jointly handle both modalities. We employ the T5~\cite{t5} Language Model for 
% To address the conditioned generation task, we employ a transformer-based model based on the architecture proposed in

with the model learning to maximize the log-likelihood of the data distribution:

\begin{equation}
    \mathcal{L}_{LM} = - \sum_{i=0}^{L_t-1} \log p_\theta \left( x_t^i \mid x_t^{<i}, x_s \right).
\end{equation}

This framework allows HOI-GPT to learn complex relationships between motion and language, enabling flexible representation and generation of diverse hand-object interactions within a single model. Our method achieves state-of-the-art performance on multiple benchmarks, outperforming previous methods by a significant margin in both HOI generation from text and text generation from HOI motion.
\\
We train the HOI language model in two stages: In the \textbf{Motion-language Pre-training Stage}, we fine-tune the T5 model~\cite{colin2020exploring, t5} on a combination of language and motion data through both unsupervised and supervised methods. By randomly masking tokens in the input, we train the model to predict these spans, enabling it to learn the relationship between motion and language from paired datasets. Following this, in the \textbf{Instruction Tuning Stage}, we construct a multi-task text-motion dataset with instruction-based prompts, covering tasks such as motion generation and captioning. This instruction tuning enhances the model's ability to generalize to unseen prompts and tasks, thereby improving its performance across diverse motion-language applications.


\myheading{Loss function.} The final training objective function is formulated as:
    \begin{equation}
    \mL = \mL_{geo} + \mL_{token} + \mL_{lm}
\end{equation}

==> sec/4_data.tex <==
\section{Dataset}  \label{sec:data}
  \vspace{-0.13cm}



